Calibrating Multivariate L\'evy Processes with Neural Networks

Calibrating a L\'evy process usually requires characterizing its jump distribution. Traditionally this problem can be solved with nonparametric estimation using the empirical characteristic functions (ECF), assuming certain regularity, and results to date are mostly in 1D. For multivariate L\'evy processes and less smooth L\'evy densities, the problem becomes challenging as ECFs decay slowly and have large uncertainty because of limited observations. We solve this problem by approximating the L\'evy density with a parametrized functional form; the characteristic function is then estimated using numerical integration. In our benchmarks, we used deep neural networks and found that they are robust and can capture sharp transitions in the L\'evy density. They perform favorably compared to piecewise linear functions and radial basis functions. The methods and techniques developed here apply to many other problems that involve nonparametric estimation of functions embedded in a system model.

==> figures/sim/sim0.75.tex <==
% This file was created by matplotlib2tikz v0.6.18.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}

\begin{axis}[
tick align=outside,
tick pos=left,
title={$\alpha=0.75$},
x grid style={white!69.01960784313725!black},
xlabel={$x$},
xmin=-124.014840327757, xmax=6.2792061373631,
y grid style={white!69.01960784313725!black},
ylabel={$y$},
ymin=-43.768189278211, ymax=75.0691250373965
]
\addplot [semithick, color0, mark=*, mark size=1, mark options={solid}, forget plot]
table [row sep=\\]{%
0	0 \\
-0.00318388555006963	0.0006246143651243 \\
0.00640099418418544	-0.0377397346890138 \\
-0.12814201151711	0.122599195965234 \\
-0.130891195979075	0.10987964887934 \\
-0.145774844350431	0.0913243831288451 \\
-0.0928139275776079	0.0864954880935884 \\
-0.0946152536752859	0.082007300530583 \\
-0.0665759951560287	0.081692315456157 \\
-0.0630536387786135	0.0789703617758829 \\
-0.0640930498191471	0.114199765075327 \\
-0.0182042852594204	0.109290833213628 \\
-0.0191293888508578	0.110338328409158 \\
-0.00564900963106567	0.102628111006957 \\
0.0120524450408572	0.0386355553358495 \\
-0.0630288204916912	0.113569808371608 \\
0.332308047952945	0.160070958215848 \\
0.334085286129059	0.162051387077659 \\
0.330300942341649	0.18854843953819 \\
0.337149023489434	0.214011738255014 \\
0.356437068739221	0.268231722136066 \\
0.356749479857634	0.263116627783987 \\
0.338795296874747	0.264235018612963 \\
0.305138234421509	0.255344980646812 \\
0.27107671609935	0.242326985429494 \\
0.245872682518915	0.21407449272013 \\
0.255379813089304	0.211683082265107 \\
-0.0173255685351626	-0.0337009613763252 \\
-0.0251148014724485	-0.0384857891861759 \\
-0.0288232504356895	-0.0053998545517975 \\
-114.784303845963	-29.4690882007567 \\
-114.773494345052	-29.4683249172294 \\
-114.793896553841	-29.4671814766551 \\
-113.712454186299	-30.0909333107889 \\
-113.71063815775	-30.0888600867947 \\
-113.71327353791	-30.0808172518811 \\
-113.720639654796	-30.0713686834843 \\
-113.729505202436	-30.0677598114971 \\
-113.737808567149	-30.1131108612966 \\
-113.642589603895	-30.1037239679965 \\
-113.889085034268	-29.9089202569389 \\
-113.878299791191	-29.9104600264029 \\
-113.915984166121	-29.9836471483824 \\
-113.894572380259	-29.967609778946 \\
-113.899861061199	-29.95823742322 \\
-113.914252313608	-29.9519645776411 \\
-113.890277284661	-29.9728304093557 \\
-113.899973496181	-29.957158403573 \\
-113.899481676932	-29.9629023740122 \\
-113.97152517647	-29.8871695300212 \\
-113.895588714619	-29.830385092019 \\
-113.819085983058	-29.7502640719703 \\
-113.800354640664	-29.7388569625988 \\
-113.778836375993	-29.7420209326684 \\
-113.785553935971	-29.7239552071507 \\
-113.768690534774	-29.7117377907158 \\
-113.701862636187	-29.6667048797488 \\
-113.690714521687	-29.6719743892048 \\
-113.615641885055	-29.7203783104026 \\
-113.632556182264	-29.7311131335384 \\
-113.429031995657	-29.6682714892966 \\
-113.489091021583	-29.6844038519239 \\
-113.951946879529	-29.6982447752623 \\
-113.950894794587	-29.7032866160883 \\
-113.977077380821	-29.7301887954149 \\
-114.124859492724	-29.8438330822649 \\
-114.123304912831	-29.8396379638394 \\
-114.127270270323	-29.8431411672832 \\
-114.475912468567	-30.5852096387445 \\
-114.465449412503	-30.5983621892031 \\
-113.193938384007	-30.4355268169259 \\
-113.219031612668	-30.157413191703 \\
-113.3319342918	-29.8661778717294 \\
-113.328729061582	-29.8673912941927 \\
-112.931485305702	-28.9695144218313 \\
-112.868650833911	-28.8495815482243 \\
-112.68896150337	-28.8217421833391 \\
-112.66496161669	-28.8297679057949 \\
-112.508025539606	-28.8265250673174 \\
-112.492284971936	-28.8170676743956 \\
-112.461053586572	-28.8036481080502 \\
-112.4495084624	-28.7981556190745 \\
-112.452813392607	-28.9239037620059 \\
-112.456243000092	-28.9262209870981 \\
-111.940531561153	-29.3359831811633 \\
-111.878614203293	-29.5432944987289 \\
-111.850214404917	-29.5722347076056 \\
-111.852911882227	-29.5800876511136 \\
-111.850786388723	-29.5803911999816 \\
-111.857307191647	-29.5828990539969 \\
-111.784713131127	-29.4898438701011 \\
-111.840570884375	-29.6028242894414 \\
-111.850331607241	-29.5996012511881 \\
-111.901936217913	-29.5651848472088 \\
-111.898402440409	-29.5857182271198 \\
-111.924601095982	-29.6055154999518 \\
-111.888057091903	-29.5795208503236 \\
-111.679203787796	-29.6527808584834 \\
-111.715413994197	-29.6573679260016 \\
-111.73098309312	-29.7234105984132 \\
-106.978130506106	-23.5722905567052 \\
-106.984123370524	-23.571794730083 \\
-107.104607708318	-23.5302841970981 \\
-107.098855058396	-23.5247817749506 \\
-107.111730008714	-23.5412950511377 \\
-107.132528209828	-23.5420083621878 \\
-107.148157889569	-23.5540806171864 \\
-107.103345852882	-23.5913951322646 \\
-107.119386411186	-23.5952312866929 \\
-107.142066626662	-23.5910483978588 \\
-103.859231384695	-23.124823698955 \\
-103.350479623131	-22.613509096015 \\
-103.317119467149	-22.616744001172 \\
-103.31597882719	-22.6189925827402 \\
-103.290290347716	-22.6159084704421 \\
-102.396503719541	-22.2589773521608 \\
-102.406397767858	-22.2586900805893 \\
-102.408810083045	-22.272960309946 \\
-102.421730778592	-22.2251850297351 \\
-102.390237353019	-22.2155546782928 \\
-102.363027178751	-22.2133398834448 \\
-102.336408286822	-22.3293824154424 \\
-101.961375709654	-22.3860989645798 \\
-101.798885342496	-21.5329162939026 \\
-102.051061984199	-21.5069486726412 \\
-102.2742741152	-21.507202912985 \\
-102.293402749118	-21.5221112406899 \\
-102.363034421635	-21.4757115309873 \\
-102.388187787329	-21.4168191926415 \\
-102.380788340308	-21.4044434979665 \\
-102.354531184334	-21.4212907832664 \\
-102.35777549179	-21.4254563754268 \\
-102.417581902542	-21.4481235088857 \\
-102.418156806758	-21.4461786868755 \\
-102.41961865108	-21.4308845661109 \\
-102.241914707027	-21.4106922056716 \\
-102.245045072328	-21.4145920960541 \\
-102.241033623065	-21.417875298455 \\
-102.234623387717	-21.408917859227 \\
-102.241112812858	-21.4086325326863 \\
-102.237945042631	-21.4051601238038 \\
-102.223614878024	-21.4027172924102 \\
-102.215662209448	-21.3205918992229 \\
-102.172323212059	-21.4733707875998 \\
-102.146611473147	-21.4311207683218 \\
-102.106633487399	-21.4183963118729 \\
-102.107768118537	-21.4135512128115 \\
-102.128362477943	-21.4262029203863 \\
-102.133475670122	-21.3621058213713 \\
-99.9380701978552	-21.3584168065155 \\
-100.307440588381	-21.4193320351871 \\
-100.350406651577	-21.413378253453 \\
-101.221846111576	-26.0549376915917 \\
-101.232264831922	-26.054846774397 \\
-101.137654612961	-26.351573102611 \\
-101.136170243245	-26.3488332846978 \\
-100.807841905869	-26.1687068887331 \\
-100.799257904791	-26.1680056283585 \\
-100.797695701483	-26.1747136021099 \\
-100.654126442395	-26.1816377820695 \\
-100.695248151055	-26.2068023538907 \\
-100.673423202447	-26.2076229422919 \\
-100.316182042321	-26.4236453635866 \\
-100.310218603668	-26.4373000460376 \\
-100.33375098726	-26.4510196384952 \\
-100.32274992129	-26.466972773226 \\
-100.3694594163	-26.4528185202301 \\
-100.34608894139	-26.4694105544788 \\
-100.249477602646	-26.5511711002857 \\
-100.212621225006	-26.5303374513043 \\
-99.9683496535185	-26.4634017759459 \\
-99.8591703291642	-26.0931292349581 \\
-99.8537688872867	-26.1138710119465 \\
-101.840676376349	-25.4588789192735 \\
-101.84806406171	-25.4596000161344 \\
-101.845142352032	-25.4584042536165 \\
-101.835387105745	-25.4321872035152 \\
-101.890686464344	-25.4977573355197 \\
-101.876505747914	-25.6074898131377 \\
-101.879803031771	-25.6266576448065 \\
-101.872827820363	-25.6146436240691 \\
-101.877155693195	-25.6127424929496 \\
-100.237321634031	-24.7084732117021 \\
-100.233917555043	-24.7258954994636 \\
-100.526747323116	-24.9833348650769 \\
-100.734675885095	-24.6740536438904 \\
-100.783315750805	-24.6798025148728 \\
-100.681035938323	-24.6724377984514 \\
-100.706604193607	-24.6619323187292 \\
-100.72417214002	-24.7268640697567 \\
-100.892084095034	-24.4508861958751 \\
-100.896824493007	-24.4428088110676 \\
-100.898283470661	-24.4002402669299 \\
-100.896138444024	-24.3991764610773 \\
-100.893552187768	-24.2728636558371 \\
-100.887351400669	-24.2692904715282 \\
-100.888421404941	-24.2681474889892 \\
-100.88920479862	-24.2684428893123 \\
-100.844371745221	-24.2446972536994 \\
-100.849690592342	-24.2502760497262 \\
-100.825543352753	-24.308220331226 \\
-100.829832831807	-24.2828013454976 \\
-100.823505649301	-24.2887782417752 \\
-100.809805561478	-24.2917570386086 \\
-100.802282503329	-24.2904534048215 \\
-100.868322448089	-24.3241521568872 \\
-100.888579757615	-24.3669082170679 \\
-100.888715658254	-24.3551109709374 \\
-100.892757409773	-24.3891637332242 \\
-101.029645506323	-24.4508692294992 \\
-100.919630980725	-24.479706406779 \\
-100.421702867346	-24.2228109943092 \\
-100.43188366679	-24.2250126249774 \\
-100.433134856351	-24.2202700674321 \\
-100.441510829775	-24.2135855741485 \\
-100.448230700817	-24.1994662743514 \\
-100.446422628355	-24.2081996755241 \\
-100.441923356533	-24.2099769605297 \\
-100.446743293575	-24.1818419618752 \\
-100.403848100149	-24.1758626467976 \\
-100.401157090073	-24.1795515014062 \\
-100.43620648648	-24.1606053287077 \\
-100.44124755036	-24.1647813032269 \\
-100.33616959229	-23.4619705423674 \\
-100.353526296474	-23.4381955338684 \\
-100.378877272851	-23.4661898509546 \\
-100.056967676696	-24.1505841714618 \\
-100.065109432829	-24.1618034382298 \\
-100.090074199204	-24.1672354907059 \\
-100.06961292834	-24.1002695373714 \\
-100.056766009959	-24.1093706843143 \\
-100.067227185703	-24.1035251936332 \\
-100.10647340247	-24.1453032173355 \\
-100.143670260451	-24.1013661824177 \\
-100.199670434331	-24.177663634282 \\
-100.212406612521	-24.1572146564893 \\
-100.207600834564	-24.1554526492781 \\
-100.253161849564	-24.14697101883 \\
-100.332739400891	-24.0547260328205 \\
-100.323407392324	-24.0719084133218 \\
-100.109134299806	-24.041968676667 \\
-100.110857284389	-24.070002319093 \\
-98.0538181505201	-23.2173710135789 \\
-98.086656678979	-23.1872422814453 \\
-98.1287496748028	-23.1970740411972 \\
-98.1299251441541	-23.2173527750978 \\
-98.5778558047888	-23.3884860219083 \\
-98.5846772659249	-23.3787750399219 \\
-98.5683748050564	-23.3864622217345 \\
-98.5479347580142	-23.3965399164808 \\
-98.9721514238095	-23.6324670381964 \\
-98.9769822774666	-23.6330655704887 \\
-98.9751755937859	-23.6271604520065 \\
-98.976428521727	-23.6150389570136 \\
-98.9508059448214	-23.6206351634193 \\
-98.9305649807793	-23.6081166745439 \\
-98.9284506918549	-23.5803879908391 \\
-98.9476779018068	-23.5727579923631 \\
-98.905266310375	-23.570968884165 \\
-98.887973344566	-23.5439171551073 \\
-98.8918924995763	-23.5387506531171 \\
-98.889293609674	-23.5269032793469 \\
-98.7735145312326	-23.5892017515543 \\
-98.7470483655289	-23.5927299998402 \\
-98.6570498446506	-23.5309928737759 \\
-98.6389330210858	-23.5284782896752 \\
-99.0071607714144	-23.1416540243019 \\
-98.7923383869234	-24.3089942232121 \\
-98.7938079016952	-24.3026744804036 \\
-98.2753358341948	-24.4107979339173 \\
-98.3100659149053	-24.4525333924265 \\
-98.5200967730406	-24.8949733132307 \\
-98.4754513785719	-24.8769434034245 \\
-98.4881783175655	-24.8775207938958 \\
-98.4933806331651	-24.8739641932392 \\
-98.4766926323746	-24.8515192020819 \\
-98.4662748170845	-24.8559878952622 \\
-98.4321904963096	-24.8655659865487 \\
-98.4157308829812	-24.8597855304773 \\
-98.3120610575437	-24.8933729917265 \\
-98.2695469256225	-24.8940594244991 \\
-98.3049710528097	-24.8758433221388 \\
-98.1849105596836	-25.0541789070208 \\
-98.1828884980668	-25.1018137571379 \\
-98.1868064223277	-25.0911457142235 \\
-98.2611552004021	-25.0992282000511 \\
-98.2481577759017	-25.0572616065794 \\
-98.2304254916636	-25.0238150799289 \\
-98.2342479995058	-24.9720623616141 \\
-98.2259783547642	-24.9843291205085 \\
-98.2270143605331	-24.9800916306658 \\
-98.2284403941301	-24.981825971342 \\
-98.252882001988	-24.9804327612462 \\
-98.2456976539066	-24.9731222399231 \\
-98.2165769719061	-24.9673408236596 \\
-98.2372989785696	-24.9772314658535 \\
-98.2470049123507	-24.9769240599459 \\
-98.2634453412993	-24.9412834468076 \\
-97.6375734873389	-24.4992144611229 \\
-97.6190049907589	-24.4865027841709 \\
-97.6204196308421	-24.4867779955257 \\
-97.6171455016428	-24.489358738897 \\
-97.6167611077552	-24.492764870712 \\
-97.571974550801	-24.4596231786885 \\
-97.5936109068021	-24.4477979734574 \\
-97.529344140783	-24.483254101676 \\
-97.6975347797864	-24.3445057728707 \\
-97.6938279787637	-24.3426195474339 \\
-97.5325057930596	-24.3521524152152 \\
-97.5232497622654	-24.3648446252357 \\
-97.5444435871869	-24.3344694409484 \\
-97.5407333128823	-24.3532926862676 \\
-97.5416964119883	-24.3263424972314 \\
-97.5137567901742	-24.3473984225546 \\
-97.5157423900672	-24.3633451812768 \\
-97.5267821191176	-24.3490011079448 \\
-97.3803223049639	-24.3145509068701 \\
-97.3701059505874	-24.2591347124277 \\
-97.3706883359239	-24.2464981599057 \\
-97.3623374096348	-24.2337187465976 \\
-97.8097982773107	-22.2409959425996 \\
-97.8198739770385	-22.2531170488933 \\
-97.8174569521003	-22.2532906617884 \\
-97.8580924347782	-22.271764182841 \\
-97.8569668110056	-22.2724710087255 \\
-97.8878855303432	-22.304401580306 \\
-98.1182796604453	-22.3678197211954 \\
-98.1313439570155	-22.3828955079866 \\
-98.1183476912756	-22.3815508367249 \\
-98.1785269587897	-22.3881381566981 \\
-98.1696316426906	-22.3747416137689 \\
-98.1784516029481	-22.3737420441143 \\
-98.2271935323485	-22.2250791190828 \\
-98.2800426685389	-22.1704811115492 \\
-98.2820639037133	-22.1802376691334 \\
-98.2748212019818	-22.1794289650116 \\
-98.2669270650705	-22.1810159862215 \\
-98.2437772988223	-22.1735178177561 \\
-98.2532614274374	-22.1647060460082 \\
-47.207203357237	-34.1330595207609 \\
-47.2289795207438	-34.2015107337017 \\
-47.2318049952809	-34.1967158172076 \\
-47.238130404082	-34.1820365086089 \\
-46.0126546366224	-34.3281789983795 \\
-46.0169690720825	-34.3336529882948 \\
-45.9816355274512	-34.3167847760532 \\
-45.6139493674953	-34.5199888201714 \\
-45.6093913902449	-34.5196895284655 \\
-45.5686465654675	-34.5031334945208 \\
-45.571067350462	-34.5081485299785 \\
-45.5063980732633	-34.4805856816256 \\
-45.5027653894809	-34.4839892804902 \\
-45.1452994876613	-35.0497020895859 \\
-45.1631708100384	-35.0474246790279 \\
-45.1637937806297	-35.0538594082557 \\
-45.0023856916456	-34.9881307640481 \\
-45.2113347111078	-34.8244404273603 \\
-45.1650456389607	-34.7940603109986 \\
-45.1818750878775	-34.8111230530609 \\
-45.3737617715229	-34.6702556817856 \\
-45.3533120405458	-34.6442467021816 \\
-45.3601336971815	-34.6460147810804 \\
-45.3683597731205	-34.6356634829544 \\
-45.3554260447422	-34.6514086232655 \\
-45.362602248221	-34.6383689371074 \\
-45.3263984009635	-34.6702082411127 \\
-45.2950986278526	-34.687891741226 \\
-45.2776670499728	-34.6516468492717 \\
-46.0670014512534	-35.4744427587947 \\
-46.0497611756902	-35.4623703642376 \\
-46.0676680773221	-35.450275072438 \\
-44.9219610635032	-36.0742800311245 \\
-44.737051181062	-36.0709525322941 \\
-44.667131556066	-36.1193803903429 \\
-44.6613568418578	-36.1011669989789 \\
-44.6336190625022	-36.2690041164134 \\
-44.6789169529001	-36.3838971648618 \\
-44.6456796204903	-36.4163336134471 \\
-44.8246597893583	-36.2054998950239 \\
-44.8237070485981	-36.2089485030398 \\
-44.7632301645486	-36.1591328253875 \\
-44.9490914312161	-36.179600814175 \\
-44.9389830607249	-36.1769125267758 \\
-44.9539216788452	-36.1294433269632 \\
-44.9860206587731	-36.1339802244947 \\
-44.9447565375593	-36.113581111585 \\
-44.9124771773727	-36.1359454817574 \\
-44.905149179298	-36.1390143675711 \\
-44.8867820597974	-36.1379140257415 \\
-44.8900304512872	-36.1366234238521 \\
-44.8712470664698	-36.0882516527587 \\
-44.9706530060452	-36.0490246262591 \\
-44.9204235871454	-36.0804726854013 \\
-45.0228110006074	-36.0403412941767 \\
-45.0263891529287	-36.0204960486197 \\
-44.9927506696789	-36.0280106924272 \\
-44.9914817202688	-36.0260331893884 \\
-44.9179844946307	-36.0881020881262 \\
-44.9204036616951	-36.0964786556072 \\
-44.9989826232343	-36.0233521539223 \\
-44.9933011310787	-36.0693473333693 \\
-44.9858629257645	-36.0701450373082 \\
-44.9964781084626	-36.0882637167595 \\
-44.9965591790908	-36.0935835581403 \\
-44.9873005466595	-36.1047060614902 \\
-44.9690677536613	-36.0635930698608 \\
-44.9674659259785	-36.0622230013094 \\
-44.9809268506306	-36.0618299180942 \\
-44.9870095756852	-36.0642773696554 \\
-44.9906704481938	-36.0536319899875 \\
-45.0200232435732	-36.0501613465573 \\
-45.0165535045866	-36.0602826942364 \\
-44.9947966899923	-36.0601946741719 \\
-45.0252368445996	-36.0305257694369 \\
-45.01509884005	-36.0438736604947 \\
-45.0155094622616	-36.0437972451828 \\
-45.0307727693278	-36.0180881022366 \\
-45.0184136294646	-36.0283634204006 \\
-45.0143867641081	-36.0287540595752 \\
-45.027088732589	-36.0828878600558 \\
-44.9866019696469	-36.0705369341712 \\
-44.9508437422013	-36.00154727713 \\
-44.9809227819747	-35.9873762382239 \\
-45.022246269573	-36.1238952579547 \\
-45.0374518413515	-36.0772974908445 \\
-45.024112189839	-36.0780447491283 \\
-45.2476342533312	-35.8851999362434 \\
-45.2481042248196	-35.8894037142566 \\
-45.2580615032884	-35.8998372985529 \\
-45.3077378709963	-35.9169741635821 \\
-45.3414349843168	-35.9402977800228 \\
-45.2868495283673	-35.8788215347152 \\
-45.2844232324435	-35.8961380445961 \\
-45.3478928406681	-35.9124111839111 \\
-45.4092321784516	-36.054951918133 \\
-45.4213378731169	-36.0574443634136 \\
-45.2276199720077	-36.0879680990209 \\
-45.2327169022792	-36.0985066510862 \\
-45.072701322911	-36.1565655664984 \\
-45.0873588941091	-36.164051533692 \\
-45.0944521294902	-36.1676601158532 \\
-45.1304904277396	-36.2027665368376 \\
-45.4815630329524	-38.1777070944997 \\
-45.5641691627572	-38.1994164916888 \\
-45.560747943311	-38.2008276947275 \\
-45.5600284399717	-38.2022731671942 \\
-45.5683320229145	-38.2087064892884 \\
-45.5460386367002	-38.198664414383 \\
-45.5826485377968	-38.2123560278286 \\
-45.5276808015615	-38.2396232323707 \\
-45.5259888130569	-38.2353149314371 \\
-45.50957104882	-38.3586494283419 \\
-45.5517261185402	-38.3664931729561 \\
-114.04699248067	69.6005404874276 \\
-114.036640884925	69.6012495847448 \\
-114.042794445899	69.6122509407133 \\
-114.229791438694	69.6674289321416 \\
-114.231606977772	69.6300448057729 \\
-114.223593339123	69.6403435188054 \\
-114.217454491529	69.6416216112621 \\
-113.732604936405	68.9539408880742 \\
-117.606903257088	69.0146502874555 \\
-117.640973555887	69.0778196226697 \\
-117.732203910412	69.1592004956508 \\
-117.699249536823	69.1685852149459 \\
-117.703942148237	69.1795037826758 \\
-117.636922767752	69.1619973772583 \\
-117.61158089294	69.1963182861967 \\
-117.770855787517	69.2109656674287 \\
-117.777212939286	69.1950442175165 \\
-117.852403974397	69.1077551535007 \\
-117.955836176147	69.0594668420513 \\
-117.939659921735	69.0127463093458 \\
-117.613681078038	68.6939961981995 \\
-117.811652844742	68.4962960754047 \\
-117.803667998944	68.5096749182399 \\
-117.813296810823	68.5118395596377 \\
-117.800662162925	68.4848108482734 \\
-117.826306738586	68.4621095450671 \\
-117.878265901972	68.4721020301454 \\
-117.901402091194	68.4305260295438 \\
-117.952425559534	68.4146247089136 \\
-117.942884124819	68.4154926743198 \\
-118.092383670252	68.3200899937382 \\
-117.905092195756	68.4341434916084 \\
-117.895617753871	68.4357260288218 \\
-117.936853635688	68.4328774576274 \\
-117.897831310577	68.301542698976 \\
-117.957299198082	68.3319372763775 \\
-117.954984234052	68.3778404576911 \\
-117.866571935168	68.1598373504504 \\
-117.85349252664	68.1799586088768 \\
-117.830617150072	68.2175713740535 \\
-117.820549796537	68.2237466474864 \\
-117.82202583721	68.2359860189639 \\
-117.824380703426	68.2329512519034 \\
-117.869133184056	68.2296103130918 \\
-117.854177481496	68.2101471225471 \\
-117.858885438542	68.2089466885015 \\
-117.958297712679	68.0996666994617 \\
};
\end{axis}

\end{tikzpicture}

==> figures/sim/sim1.5.tex <==
% This file was created by matplotlib2tikz v0.6.18.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}

\begin{axis}[
tick align=outside,
tick pos=left,
title={$\alpha=1.5$},
x grid style={white!69.01960784313725!black},
xlabel={$x$},
xmin=-4.78609777842756, xmax=2.3807011611237,
y grid style={white!69.01960784313725!black},
ylabel={$y$},
ymin=-13.825231709635, ymax=1.42796083598013
]
\addplot [semithick, color0, mark=*, mark size=1, mark options={solid}, forget plot]
table [row sep=\\]{%
0	0 \\
-0.0828566932134131	-0.00645109559474828 \\
-0.0360092062193371	-0.185873573513541 \\
-0.202320398472258	-0.26016799828408 \\
-0.213763342313863	0.108919956285122 \\
0.0655715647340436	0.175279621538862 \\
-0.511686472011291	0.467842706346545 \\
-0.497252998335085	0.257860938824015 \\
-0.321565958711782	0.437366353753818 \\
-0.561433113611284	0.267791241629468 \\
-0.638692327597146	0.167392403016729 \\
-0.583451077593921	0.127054083668031 \\
-0.218176788642385	0.062988771948441 \\
-0.386178166643001	0.247906867756361 \\
-0.458684080267847	0.0613134729753714 \\
-0.540014902759734	0.0782606328012483 \\
-0.573348077855943	-0.11794792988138 \\
-0.618246739932856	-0.104437905337335 \\
-0.6271286281381	0.0639977427991807 \\
-0.61209658406127	0.289198751579821 \\
-0.499622944233524	0.439158159673899 \\
-0.686465481265409	0.690954522545151 \\
-0.793714730690686	0.734633902088532 \\
-1.14531547557902	0.410851059986216 \\
-1.20539514473938	0.315634719877281 \\
-1.23649812168506	0.04216064810968 \\
-1.2404424875586	0.0193169971233749 \\
-1.01021294115701	-0.0676446302774637 \\
-1.41568478810894	-0.390529237050907 \\
-1.45063814351961	-0.454438327794268 \\
-2.38246436451624	0.0449729048457972 \\
-2.33143489194662	-0.018581839383357 \\
-2.15737481579911	0.205666569534349 \\
-2.35782412460166	0.294488082175205 \\
-2.76345567002306	-0.352661299972711 \\
-2.90476793466576	-0.157421394265445 \\
-2.82096641884205	-0.350814834825612 \\
-2.6856105368224	-0.384386038775903 \\
-2.57879457432699	-0.37839876840675 \\
-2.34429769581355	0.0681282619237679 \\
-2.36889655635016	0.1612130813401 \\
-1.64541470783882	0.376401956385082 \\
-1.79185057065924	0.353279834616289 \\
-1.80078188363817	0.01351813960723 \\
-1.95386161870653	0.378530498436915 \\
-2.20180091316922	0.426196847300309 \\
-1.87208189470942	0.266864301236628 \\
-1.92031649661688	0.416593015201163 \\
-2.056238266684	0.428283776480281 \\
-1.98604440079695	0.168137602809818 \\
-2.00234682997134	0.0768292626924727 \\
-1.95573721004717	0.114352269289047 \\
-1.83908920911198	-0.00169492922989076 \\
-1.61798636659216	0.160394876739221 \\
-1.92857278634721	0.177698172034695 \\
-1.99288273696465	0.13154142666222 \\
-1.93659504140653	0.0922026182463422 \\
-1.76133996641398	0.303377082385492 \\
-2.27201992240363	0.355632261480584 \\
-2.09111537700821	0.271809789323041 \\
-2.36128297285993	0.237850705382394 \\
-2.2925269410974	0.158823484956906 \\
-2.44159959824259	-0.146584068417538 \\
-2.23237174206748	-0.530458507914843 \\
-2.19208866932641	-0.624943836207669 \\
-2.00278648121848	-0.857788915533612 \\
-1.96804686687668	-1.06864187362348 \\
-2.05007331147494	-1.09597777563172 \\
-2.05839349663048	-1.2794679009989 \\
-2.23211217684232	-1.36746388208475 \\
-2.28932875418897	-1.49227329348424 \\
-2.18751110087961	-1.64453518203784 \\
-2.37445171397066	-1.43274649243928 \\
-2.5016791408347	-1.44265890654721 \\
-2.73437359751532	-1.36362755934531 \\
-2.84430583993712	-1.43799939713377 \\
-2.90192491233959	-1.5451087059531 \\
-2.61915964465848	-1.45507973165313 \\
-2.7466430179551	-1.49989051869803 \\
-2.54469557237565	-1.594851924695 \\
-2.65710469640197	-1.312350397634 \\
-2.75025075529889	-1.41381531836399 \\
-2.82671144361892	-1.68898750001755 \\
-2.89047648287774	-1.8657036628586 \\
-2.62421008715395	-1.55753748743049 \\
-2.68736511077621	-1.66664144386511 \\
-2.7108056302381	-1.77465855816714 \\
-2.76288514765216	-1.61019311426983 \\
-2.76471923893328	-1.82065868167434 \\
-2.57839504195025	-1.73100013833466 \\
-2.52783355114574	-1.84802456684172 \\
-2.34085279803923	-1.77233302337213 \\
-2.39175873267154	-1.73814186354316 \\
-2.11977958875934	-1.35577010659876 \\
-1.94445710940138	-1.44092949150801 \\
-1.89720942945043	-1.59584617907316 \\
-1.92971083535535	-1.41697210055456 \\
-1.96442829193187	-1.55014954965631 \\
-1.75581071962264	-1.47916802959117 \\
-1.55444902697258	-1.58384836722574 \\
-2.1259607696148	-1.46810785345616 \\
-1.87882414801561	-1.40579625969484 \\
-1.96665006022072	-1.23234019304953 \\
-1.96559803087742	-1.33598964229627 \\
-1.82866742207644	-1.3889432601403 \\
-0.7936824365536	-0.89424268249672 \\
-1.05277811769959	-0.664796977589179 \\
-1.16120263428707	-0.67699677528542 \\
-1.2350938483879	-0.815496286964954 \\
-1.42294738101856	-0.811461584404666 \\
-1.66275715745254	-0.846907534141829 \\
-1.66336888875674	-0.813582308499928 \\
-1.66067683320686	-0.828314183495643 \\
-1.59219596137669	-0.692082704689896 \\
-1.65223833921147	-0.782677557429528 \\
-1.59770292945646	-0.826162156149484 \\
-1.76012420810469	-1.29974352984541 \\
-1.86939638859957	-1.47136573434219 \\
-1.9463456363158	-1.56844137307117 \\
-2.20569370610352	-1.23373786387505 \\
-2.17523199997095	-1.14669870131581 \\
-1.87660697451464	-1.05793703127393 \\
-1.90281976366659	-1.07629134577097 \\
-2.05225079014119	-0.924930064650236 \\
-2.06142929036457	-0.905099004426612 \\
-2.27669441595348	-1.07229991325691 \\
-2.50731067074382	-0.935980340776501 \\
-2.47086417652886	-1.00608763585071 \\
-2.15571373862122	-0.989282811648839 \\
-2.15271959366916	-0.883396874623586 \\
-2.79164792097959	0.0837338665020737 \\
-2.78842140617979	0.190099199499998 \\
-2.90776451322163	0.296876280784957 \\
-2.98978092961834	0.171567663397356 \\
-2.88958594657463	0.0287515225775061 \\
-2.98031822826319	0.00785748434970766 \\
-3.02438179995195	-0.0589841197499182 \\
-3.00279948254562	-0.113226980030398 \\
-2.83772662787701	-0.104838919751174 \\
-2.83441086205128	-0.281395078731669 \\
-2.88871053416026	-0.456248367492086 \\
-2.86127908366376	-0.308897996762682 \\
-2.6131765754337	-1.22242662636573 \\
-2.52489469218552	-1.30306521590137 \\
-2.93549346976286	-1.37127800605691 \\
-2.94245266194884	-1.3473164483216 \\
-3.13610691203985	-1.22054952077055 \\
-3.50602818315207	-1.11625189379145 \\
-3.7813459141612	-6.86573910529135 \\
-4.15090383768559	-6.69293550720002 \\
-4.09122571740372	-6.72837092692462 \\
-3.86344995656049	-6.71441250235664 \\
-3.37713075839181	-6.65543667608331 \\
-3.72800556132019	-6.59625068404042 \\
-3.63752872981044	-6.41053950189335 \\
-3.57667782334027	-6.25842800152327 \\
-3.38803822681583	-5.98079340199011 \\
-3.45957510424946	-5.91573571540966 \\
-3.48503587063801	-5.73601817373857 \\
-3.14738226669964	-5.70180762832787 \\
-3.02532981176686	-5.55945712754687 \\
-3.06403530019961	-5.45410944787074 \\
-3.17353616232573	-5.64075275475975 \\
-3.21292901388684	-5.50089373037545 \\
-3.24196737115627	-5.35476246716935 \\
-3.10546352100075	-5.5128601277579 \\
-3.08393511072137	-5.73177294186039 \\
-3.03940576973694	-6.88728337246765 \\
-2.95764350319405	-7.06499083384801 \\
-2.84602777027572	-6.98911217116501 \\
-2.83733140532022	-7.14334147667754 \\
-2.69973533879462	-6.97753888633621 \\
-2.666606113364	-6.91657252554544 \\
-2.69248505997886	-6.88096660460457 \\
-2.74089231892196	-6.92513964769892 \\
-2.88804253236506	-7.16698474842958 \\
-2.9970118397397	-7.2039931302987 \\
-3.30229317397399	-7.42372413394257 \\
-3.6323779311143	-7.53952950849425 \\
-3.66064741443883	-7.60542826864364 \\
-3.91558891868344	-7.59657635184134 \\
-3.79793134750926	-7.55801069760725 \\
-3.76981894366528	-7.48046479731282 \\
-3.7440563479031	-7.45531367024356 \\
-3.7607812776123	-7.45945490812607 \\
-3.78704064218318	-7.30930304849122 \\
-3.85121575072856	-7.14916260202862 \\
-3.82391386327618	-6.98721815951106 \\
-3.83108832736456	-7.34277710357045 \\
-3.80379765086037	-7.31506176502046 \\
-3.93454836848773	-6.93365708575345 \\
-3.75246312605089	-6.97016510038436 \\
-3.87075734690394	-7.03105882125515 \\
-3.96175105327102	-6.72648236735645 \\
-3.78635467792831	-7.1316992906298 \\
-3.50624439709596	-7.22689060891229 \\
-3.57711363840133	-7.23493184930993 \\
-2.05594851895199	-6.62184547795167 \\
-1.96261781243981	-6.75431460120944 \\
-1.90520079893256	-6.70928295246952 \\
-2.02819913495064	-6.67571280047499 \\
-2.08779734337771	-6.73909592801981 \\
-1.88213453230976	-6.63379981289104 \\
-1.81761992856079	-6.75300880768033 \\
-1.30993736843906	-6.59598231752726 \\
-1.30245743124511	-6.57864587810083 \\
-1.29908346729019	-6.73673932663924 \\
-1.38593461826424	-7.85679935988808 \\
-1.44300727614188	-7.62265482790305 \\
-1.49636420642394	-7.31287414502222 \\
-1.54292559216757	-7.49200708152191 \\
-1.36699481805045	-7.56630774371072 \\
-1.39723667501312	-7.46101181774789 \\
-1.48051152203421	-7.30992116500016 \\
-1.53144159561408	-7.5478111212254 \\
-1.69796810825378	-7.57320047883571 \\
-1.70864803013399	-7.61821099149603 \\
-1.68174458955332	-7.52064973627777 \\
-1.81878049752952	-7.37765316074618 \\
-1.97624601646577	-7.35911655728491 \\
-1.77076652651056	-7.29231810370858 \\
-1.60256961882963	-7.29916685443275 \\
-1.52589416554133	-7.23673860247952 \\
-1.14975570860443	-7.24244512250061 \\
-1.29814227156289	-7.39429805349917 \\
-1.26825277266789	-8.00980590952212 \\
-1.69993207755384	-8.1265638285507 \\
-1.78642233373669	-8.2662266487662 \\
-1.7871811837941	-8.27728600305836 \\
-1.90207544158273	-8.32033922292154 \\
-1.95607965064984	-8.447147396917 \\
-2.12576273696379	-8.52849545944046 \\
-2.03400815340342	-8.39605172475411 \\
-1.96934905301569	-8.71407421540964 \\
-2.03721124060797	-8.68875914258241 \\
-2.1120687349482	-8.59151392028902 \\
-2.08172808812593	-8.52834895995861 \\
-2.25692018119901	-8.30294446704966 \\
-2.22889812074849	-8.40699904350688 \\
-2.38885984562508	-8.40112255945886 \\
-2.50820504906061	-8.33530225052493 \\
-2.25494575480765	-8.38941178664267 \\
-2.47243858318692	-8.34485242826342 \\
-2.60565703823704	-9.00060446614821 \\
-2.14291400755778	-8.83422171203922 \\
-2.09758220209987	-8.9680432076032 \\
-2.33410935345705	-13.1319047757434 \\
-2.45530174066458	-13.0978814581935 \\
-2.49089915556437	-12.8136378735188 \\
-2.46657953863525	-12.7278267001962 \\
-2.62942517807311	-12.6330404273306 \\
-2.6569683924963	-12.8969307639418 \\
-2.67469741509459	-12.7871142012891 \\
-2.993919294526	-12.3130606455258 \\
-1.94608923131683	-10.6776294651022 \\
-1.75483840856706	-10.6875159721419 \\
-1.85902624450888	-10.822146093331 \\
-1.94708258266529	-11.004163551496 \\
-1.59166396928798	-11.0800319657031 \\
-1.52818723975674	-10.9697032829458 \\
-1.76517320082664	-10.7787773546644 \\
-1.27909618804163	-10.5517877735606 \\
-1.39125688340938	-10.2928589748939 \\
-1.52681771665794	-10.214162215832 \\
-1.51729430278462	-10.4868473378094 \\
-1.47663348385287	-10.3842247220661 \\
-1.63732800941022	-10.1730138442206 \\
-1.67135703265795	-10.2523916768241 \\
-1.7821962080312	-10.174420688951 \\
-1.88244595034835	-10.0259516045873 \\
-2.11926188131758	-9.92820818253255 \\
-2.16958678505294	-9.89137503102272 \\
-2.202460523371	-10.0510062453991 \\
-2.17181831306377	-10.0914437699284 \\
-1.90152902695931	-10.0604202706081 \\
-1.95112641140539	-10.1638866875359 \\
-2.021743683064	-9.95931688007805 \\
-1.88348827411114	-9.93941098372562 \\
-2.27916600215613	-9.91402953925466 \\
-2.2403424609907	-9.88134348816014 \\
-2.23253426088548	-9.9035538342136 \\
-2.24914815228256	-9.75565506091067 \\
-2.29977727997923	-9.80463730165203 \\
-2.28245651528094	-9.95874404631617 \\
-2.32810218243377	-10.0035118632306 \\
-2.29530780811115	-10.1598022673284 \\
-2.4121079655606	-10.1569851127284 \\
-2.30448554193155	-10.1586982647817 \\
-2.38571237111081	-9.94452283321457 \\
-2.82872885644984	-9.53811505109245 \\
-2.73097932122739	-9.66526643001149 \\
-2.64354316980493	-9.52595646950395 \\
-2.71604489202039	-9.91274372809055 \\
-2.58840835781898	-10.0981999455304 \\
-2.49994382456693	-10.0406907671394 \\
-2.37079884588534	-10.0767469837075 \\
-2.26010680064256	-10.3953611608269 \\
-2.37514106675748	-10.4687190103172 \\
-2.43232241041	-10.1020064989307 \\
-2.60097866478539	-10.3453911822967 \\
-2.64772112155894	-10.1982155054264 \\
-2.81508770179734	-9.657549933215 \\
-2.60780651703718	-9.50508600477871 \\
-2.52410389891332	-9.64372552690837 \\
-2.88430841332772	-9.59933761419036 \\
-2.85035737701874	-9.76369584464756 \\
-3.26369524063526	-9.95210391725394 \\
-3.22730580602913	-9.95128224970496 \\
-3.39408230602715	-10.0484783731169 \\
-3.4199348663931	-9.95066451076043 \\
-3.44041759520439	-10.1111998574628 \\
-3.35281814467902	-9.99703588818545 \\
-3.42254388708108	-9.76187785227416 \\
-3.58738677280291	-9.73821035445206 \\
-3.71802591773303	-9.73310236882799 \\
-3.86871202239426	-9.70855392062182 \\
-4.1864096786762	-9.58515093946426 \\
-4.25633553629584	-9.74795240238637 \\
-4.23933038559991	-9.67175842197767 \\
-3.79566858902632	-9.23320714645653 \\
-3.75146820907901	-9.51785266528572 \\
-3.67383335595871	-9.49817334645181 \\
-3.45471166431793	-9.68506901989814 \\
-3.45894410978474	-9.87459792102057 \\
-3.67010836835238	-9.50943880493598 \\
-4.028985148445	-9.60441674716993 \\
-3.97674127584119	-9.61074756681278 \\
-4.06825101036237	-9.73862673217688 \\
-4.25385099138152	-9.66008613192766 \\
-4.03968837196501	-9.50664572932668 \\
-3.98654882914339	-9.45631738474192 \\
-3.98981861756162	-9.46372321349091 \\
-3.91744423366863	-9.34278487524073 \\
-4.09520990411591	-9.28939661272388 \\
-3.96718536207961	-9.31410966489934 \\
-3.92021731054138	-9.42734485317123 \\
-3.9595638768613	-9.47280823102804 \\
-3.90630872085031	-9.45341879664008 \\
-3.88190378558532	-9.18379229682819 \\
-4.0661960768546	-9.11964584625525 \\
-4.23436099624003	-9.08087345186349 \\
-4.23096528497713	-8.76037057085452 \\
-4.10641670846479	-8.57693725141009 \\
-3.94827565250536	-8.39847298129759 \\
-4.06732339409656	-8.33544809765363 \\
-4.16594926259686	-7.97300986931208 \\
-4.22416221897915	-8.1197513603207 \\
-4.27766558415292	-8.01722701690807 \\
-4.37511019640891	-7.97843335511019 \\
-4.46033419026614	-8.04015478320732 \\
-4.30414704884523	-7.52934074568013 \\
-4.21245950997311	-7.59042109463232 \\
-4.34204671979885	-7.5042711994809 \\
-4.26612938869717	-7.57887529494894 \\
-4.2883769267043	-7.58443685958836 \\
-4.28950703951969	-7.70348993601045 \\
-4.20373261815607	-7.85669401066991 \\
-3.95171740197489	-8.20523397456281 \\
-3.97016273401396	-8.35159190908522 \\
-4.18473193552387	-8.25182867688872 \\
-4.33591190501331	-8.4425059057347 \\
-4.21985975103968	-8.2886219056748 \\
-4.33609111908838	-8.27563135569675 \\
-4.11593937366759	-8.22251551703655 \\
-4.04355048627496	-8.11768516344063 \\
-4.17001520689952	-8.36724734183897 \\
-3.99905948254868	-8.35045269422578 \\
-3.9285160634124	-9.18181546545425 \\
-3.96491583975967	-9.18298004583798 \\
-3.90547592879477	-9.23766483141982 \\
-3.87478177124817	-9.34450155948329 \\
-3.86055106810394	-9.11787714237333 \\
-4.00339811874419	-9.10651856837473 \\
-3.91772662331217	-8.91313595360823 \\
-3.98408730390211	-8.92173652010761 \\
-3.63313094987296	-9.51817349674687 \\
-3.70862782869113	-9.71826066000967 \\
-3.72879666776924	-9.76173756356027 \\
-3.60550172253018	-9.88369099958235 \\
-3.58596182960788	-9.88089809813784 \\
-3.58729234354871	-9.84508135919637 \\
-2.87253814112025	-10.7319925758474 \\
-2.90370267938055	-10.8515341957956 \\
-3.02900275116451	-11.0869772281329 \\
-3.10081753638777	-11.0066314277742 \\
-3.90274920056335	-11.4407788649219 \\
-3.87310385814384	-11.4219598784038 \\
-3.72061978370746	-11.8822653958085 \\
-3.63953369010246	-11.7326968459622 \\
-3.85205503851639	-11.816501811687 \\
-3.82111391571636	-11.7166301768209 \\
-3.81538783889791	-11.633939544309 \\
-3.74450282254303	-11.6774291394312 \\
-3.70427716759008	-11.5736426020805 \\
-3.85553705828214	-11.6492911327731 \\
-3.73957401876875	-12.2228266469701 \\
-3.41013423431608	-11.7777935783578 \\
-3.34336453143897	-11.9002055288908 \\
-3.44782840549466	-11.856246944459 \\
-3.83185332297044	-12.1453997647363 \\
-3.81934190334495	-12.0321265739967 \\
-3.77341647981787	-11.974570388441 \\
-3.25806823302123	-11.7939242677321 \\
-3.0702751060377	-11.7542252010306 \\
-3.00045455063564	-11.6747714747436 \\
-3.13364539924262	-11.6170631552429 \\
-3.20097961636989	-11.6764227382997 \\
-3.17582348184558	-11.7446337055914 \\
-3.03349871735519	-11.5309508779902 \\
-2.84312779594389	-11.6102071583085 \\
-2.88871155414885	-11.5976026612797 \\
-2.9446106476318	-11.6836948138542 \\
-2.8126866147705	-11.6873667795 \\
-2.56629819047321	-11.9625164926655 \\
-2.44219548990829	-11.9047898121036 \\
-2.35056536110889	-11.8541323168794 \\
-2.01094287443925	-10.8526565318551 \\
-2.10340667940495	-10.6910632464723 \\
-1.97915711186955	-10.9870549400924 \\
-2.08690966381611	-10.9869581905458 \\
-2.05346274811596	-11.1098161601113 \\
-1.96647816620253	-11.223930283661 \\
-1.82992960890778	-11.0988418042979 \\
-1.83680021218517	-11.0797492179749 \\
-1.50857589956875	-11.4488117076545 \\
-1.43857528543558	-11.3364498905231 \\
-1.40355766659225	-11.4772909842513 \\
0.655034845329825	-7.16614481306397 \\
0.480185484780548	-7.42161116795112 \\
0.508229247835481	-7.48850754638387 \\
0.434099070285887	-7.5335272970927 \\
0.309898738868414	-7.58540682300542 \\
0.16218278994548	-7.53770440383988 \\
0.0823851371156404	-7.40859011529566 \\
-0.152723290898555	-7.27969635751505 \\
1.24265004530709	-6.75095736768302 \\
1.36069291234354	-6.55470280141455 \\
1.48853038931018	-6.60682262417206 \\
1.55559733722481	-6.67649953957123 \\
1.56968764384827	-6.61024509797491 \\
1.45766578725062	-6.52117157341064 \\
1.52095474797339	-6.6190744617117 \\
1.5738739015105	-6.69106344571359 \\
1.82096740393034	-6.99140590891352 \\
1.95549218301895	-7.20029245369254 \\
2.01309188516332	-7.34638637022926 \\
2.05493757296228	-7.48421941769261 \\
2.04535788643315	-7.41936256299828 \\
2.04801793005297	-7.52671483091591 \\
1.79623158450694	-7.70585007912846 \\
1.72811138551358	-7.78761347374037 \\
1.07847342024709	-8.12546580874714 \\
0.945527300714631	-8.22933985648628 \\
1.27554888318362	-8.23410327430837 \\
1.03655242956661	-8.13211785359312 \\
1.16219094517044	-7.89723841243211 \\
1.09903069740134	-8.08438578757557 \\
1.11105782885346	-8.43348774490018 \\
1.26847374666792	-8.47106032168473 \\
1.34561700956766	-8.42183833713586 \\
0.932893266213052	-9.702974619106 \\
0.984335900086065	-9.81002419064064 \\
1.14362782642641	-9.78249587871756 \\
1.02955422546798	-9.84367468543891 \\
0.911787543970406	-10.041112910763 \\
0.758765216890101	-10.4558649166414 \\
0.796316906105229	-10.38242494851 \\
0.953801437549787	-10.6072985997382 \\
0.98422311131825	-10.5979722327058 \\
1.20603605436617	-10.7619490387509 \\
1.23790863650516	-10.6992070204848 \\
1.40956696039945	-10.8683409954245 \\
1.1627828530776	-10.920188830677 \\
1.22147469130743	-10.7838574564721 \\
1.60614489355045	-11.109889093806 \\
1.47502100304679	-11.0291516249196 \\
1.50783363289395	-10.7771434679035 \\
1.43020145154877	-10.7473614458432 \\
1.09939484287149	-10.8366139623387 \\
0.8798782578291	-10.5510742900557 \\
0.789919189735534	-10.3219502858071 \\
1.03034687256911	-10.345053048057 \\
0.827967697466393	-10.2820588454519 \\
0.875335459479461	-10.1315267042666 \\
1.03647001139022	-10.2010243489151 \\
1.06577809291372	-10.1780450962389 \\
0.77241618532659	-10.0127531215219 \\
0.923833589400856	-9.97379637559456 \\
0.907269313865538	-10.2388901118483 \\
0.968991251225154	-10.2995220157415 \\
0.992526336558218	-10.2118789676994 \\
0.74661905546124	-10.0702464581996 \\
0.649443868264478	-10.1082260237671 \\
0.622951977052846	-10.3573804495396 \\
0.570817671446648	-10.1576028420983 \\
0.586351416549838	-9.96542358696561 \\
0.416071101160806	-9.91417414859311 \\
0.540252307840458	-9.88135948051064 \\
0.515024369034744	-9.86833456156883 \\
0.65811459493236	-9.97110522184536 \\
};
\end{axis}

\end{tikzpicture}

==> figures/sim/sim2.0.tex <==
% This file was created by matplotlib2tikz v0.6.18.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}

\begin{axis}[
tick align=outside,
tick pos=left,
title={$\alpha=2.0$},
x grid style={white!69.01960784313725!black},
xlabel={$x$},
xmin=-7.64869604826994, xmax=1.08742324157996,
y grid style={white!69.01960784313725!black},
ylabel={$y$},
ymin=-0.633323492951205, ymax=13.2997933519753
]
\addplot [semithick, color0, mark=*, mark size=1, mark options={solid}, forget plot]
table [row sep=\\]{%
0	0 \\
-0.28576778490985	0.245122493631188 \\
-0.767361941571711	0.840736269747897 \\
-0.600505337818707	0.728043066377132 \\
-0.097430506798751	0.785360765663089 \\
-0.0275225058938088	0.577117924187762 \\
-0.108068532441784	0.672122474536362 \\
-0.0716623932988688	1.15739550584699 \\
0.444083750929271	0.827069091154681 \\
0.584614493050038	1.03050790774691 \\
0.606512250974942	1.5096904959506 \\
0.591476884558462	1.08195909595402 \\
0.5720829195779	0.893530265013131 \\
0.500276387307549	0.122799991276775 \\
0.648136818922339	0.233285814518855 \\
0.690326910223148	0.357562407218548 \\
0.236311360605324	0.338367833450486 \\
0.20002480628299	0.563156494109597 \\
0.137577901095713	0.456161001261264 \\
-0.0795297040179525	0.170393653365161 \\
-0.237405309597531	0.562485620433728 \\
-0.418535898571667	0.944533047251643 \\
-0.576711656294879	1.15989152781471 \\
-1.23226798894597	1.2967950223426 \\
-1.46137910537159	1.3427939170265 \\
-1.4339950370325	1.2490602041577 \\
-1.2092380971507	1.52641653205486 \\
-1.31686852224785	1.5890961152061 \\
-1.47158125410212	1.59736328189739 \\
-1.58675807016556	1.38929904314645 \\
-1.68254962038787	1.39620336549658 \\
-1.85995642362022	1.72495627228069 \\
-1.85752958833929	1.82578484124497 \\
-2.37364377583132	1.77888761699057 \\
-2.58046227919363	1.88740731520532 \\
-2.62744255372903	1.84680423750192 \\
-2.5496633290124	2.13073185651007 \\
-2.70188001064323	2.34579315795379 \\
-2.50403633895744	2.31010473734411 \\
-2.52558473534375	2.31154532082737 \\
-2.5944157989094	2.49214082468506 \\
-2.48838953808393	2.46806787823214 \\
-2.40863202855128	2.66106815849259 \\
-2.8139349010826	2.64517528347598 \\
-2.49208020377403	2.98782858470011 \\
-2.52850151515379	2.96647825636496 \\
-2.54033439219301	3.33625633838044 \\
-2.67971879194604	3.25774039913384 \\
-3.17469140219022	3.11083850154828 \\
-3.29194413602573	3.55307800785718 \\
-2.84115843068472	3.85719549712121 \\
-2.669176426997	4.18661881828914 \\
-2.22604407435606	4.352308116221 \\
-2.21804963247728	4.32988834377395 \\
-2.12656668247363	4.09425982265692 \\
-2.07561239716509	3.6061701850324 \\
-1.92845652137204	3.69821981993796 \\
-2.19530951430989	3.80591753471303 \\
-2.25271108446483	3.78835773826092 \\
-2.44465627187532	4.03623024999938 \\
-2.22967805003266	3.99379945062188 \\
-2.66089941731531	4.06479865679572 \\
-2.66807157521406	4.04934617757246 \\
-2.78429322419021	4.54809648858299 \\
-3.46948492765362	4.00427023081733 \\
-3.51785975906303	3.98272022109275 \\
-3.25625927130614	4.09676167737347 \\
-3.20184232047404	4.30443912665603 \\
-3.20951905836202	4.21171202520111 \\
-3.23727794791131	4.79020380213372 \\
-2.99596797973972	5.02584626908344 \\
-3.33890505436688	5.06124675835154 \\
-3.10959444021545	5.30386412951992 \\
-3.37590376665418	5.08514339879572 \\
-3.0730760185239	5.34345600478422 \\
-2.82932744742065	5.67169485021327 \\
-3.32839685893636	5.95451822557931 \\
-3.71273175828909	5.90827339594099 \\
-3.50840412744211	5.92969000461101 \\
-3.51948893374665	5.92575655299247 \\
-3.26002562001423	5.48221944835529 \\
-3.2300030846246	5.39358278839652 \\
-3.22022311615522	5.43174516748545 \\
-3.30336404728564	5.23029080738506 \\
-3.4528401238841	5.60183626724523 \\
-3.55573591322105	5.82648930309954 \\
-3.51219021506354	6.04755334348381 \\
-3.32025910165619	6.33980189480841 \\
-3.19782786470863	6.45738480355023 \\
-2.84466013539882	6.06129995502819 \\
-3.23398741372232	6.6702750688044 \\
-3.2017965107911	6.7113775676672 \\
-3.05215418425142	6.14026573348745 \\
-3.15550322939768	6.26901840031357 \\
-3.61626144910976	5.8638301588794 \\
-3.75067008109249	6.01658274942567 \\
-3.53609313590179	5.91884988725279 \\
-3.5561317768	5.897193876298 \\
-3.15061834106259	5.8922544084709 \\
-3.08943786578493	5.76378561104794 \\
-3.54832927015863	5.65337133113071 \\
-3.87691643665577	5.74876584532021 \\
-3.83107006194752	5.86571822784337 \\
-3.88118673534074	5.67890479484577 \\
-3.5654700647286	5.50213101465033 \\
-3.87410003297825	5.49638035191838 \\
-3.93865528938757	5.59504174986044 \\
-3.91611321679784	5.70495877444209 \\
-4.35644105245629	5.97686313592096 \\
-4.60039791430613	6.20138775371811 \\
-4.6912388012549	6.50276540696183 \\
-5.07987711689807	6.02799494211552 \\
-5.04210572535534	6.03977650110376 \\
-5.28131744433038	6.0050512704329 \\
-5.36428566633541	5.93825606424915 \\
-5.23532662825489	5.90576054009802 \\
-5.08246376033873	6.01787025941138 \\
-4.88306746719247	5.91253142692768 \\
-4.39240864591149	5.87708683192835 \\
-4.56998634806309	5.39142866274511 \\
-5.13540845254292	5.30051250674271 \\
-5.19593215912024	5.51253241301775 \\
-5.20306056235218	5.89733955413492 \\
-4.81123885403762	5.82502409162675 \\
-4.78229184967073	6.10286832740483 \\
-4.52403346945708	5.99760138507589 \\
-5.01992558370025	6.09952821542929 \\
-5.09314539876196	6.45535025743017 \\
-5.16219246800067	6.42437498546161 \\
-5.1231362649318	6.53589302704438 \\
-4.74459439007835	6.18552940001554 \\
-4.40703433959059	5.79468065120664 \\
-4.88431696602345	5.96247832982222 \\
-4.80859030473698	5.71956909992496 \\
-4.70499607573749	5.62891114181101 \\
-4.74190571634964	5.72899687612158 \\
-4.91682294816924	5.71952635499021 \\
-4.7067448712368	5.72370581395838 \\
-4.98068742241182	5.5672669080695 \\
-4.70132757578593	5.64299129003547 \\
-4.58352539380581	5.75459918592557 \\
-4.49615024127504	5.54678091494171 \\
-4.42298343160542	5.35306215378862 \\
-4.62526439519262	5.25162626579368 \\
-4.50356277046322	5.1250913927248 \\
-4.9329459799476	5.12235298256753 \\
-4.65247068181279	5.35941796853673 \\
-4.52986307980018	5.40777365846686 \\
-4.25610458090564	5.54063611635811 \\
-4.21955763085916	5.30357662187609 \\
-4.66107644474087	5.58456540766094 \\
-4.96896985494455	5.41378414113231 \\
-5.29167572176636	5.33346487634539 \\
-5.04010108215631	5.02236008304675 \\
-5.11609832342901	5.06991085210158 \\
-5.02643799569419	4.67441171410997 \\
-5.15681968533251	4.83019424857348 \\
-5.22546368173092	4.88974035573431 \\
-5.73060218869298	5.10459298677272 \\
-5.81289385833673	5.10666537980211 \\
-5.50893794532875	5.31131110828306 \\
-5.59232095364438	5.27681504361378 \\
-5.71016939606475	4.65523924859247 \\
-5.6866866930454	4.75294677340938 \\
-5.67171075370106	4.8349950532267 \\
-5.42975930487933	4.37068405096785 \\
-5.2394564017126	4.70396762178579 \\
-5.10711007864714	4.50875474321493 \\
-4.82003790680875	4.19136203012571 \\
-5.14581101981118	4.27409991905186 \\
-5.37210037448023	4.42763142935847 \\
-5.1782095813178	4.46958039922002 \\
-5.46152793998984	4.43568876838821 \\
-5.25533165011243	4.00772832500952 \\
-5.30423647321072	3.74176841036207 \\
-5.2852546127161	3.72349177879645 \\
-4.89704790620066	3.78452912266241 \\
-5.15240434945117	4.04655870250713 \\
-4.86102621894086	4.33755779490738 \\
-4.97992255566255	4.20299365152951 \\
-5.15093708561792	4.21495659691721 \\
-5.32459471015658	4.12531148882899 \\
-5.52195684189965	3.79636434757873 \\
-5.74477165324238	3.80866413560643 \\
-5.60449904544295	3.93208405330003 \\
-6.27360708508817	4.06424443298249 \\
-6.05424304108998	3.95206101884186 \\
-6.43065874051074	3.92371479397006 \\
-6.12561940646864	3.66616488354144 \\
-5.52142588128208	3.63067988115031 \\
-5.56991292822697	3.69312883879505 \\
-5.22312823341126	3.49022830445641 \\
-5.47291982721034	3.64079024761243 \\
-5.28391697493479	3.58648129596755 \\
-5.23755648455067	3.57700244005733 \\
-5.01056113309147	3.86049748825695 \\
-4.86895078512877	3.77409788590651 \\
-4.36990261565734	4.07935793519162 \\
-4.7407642561044	4.12582632706667 \\
-4.23194381543306	4.27352562836418 \\
-4.25754776236912	4.17444206513983 \\
-4.43078196006105	3.79666499541619 \\
-4.4190393839696	3.74549424998341 \\
-4.51275976413541	3.88451522113733 \\
-4.52316437946375	3.66440185974104 \\
-4.69446514273411	3.52822058969541 \\
-4.84838693306446	3.38974723268058 \\
-4.8308030193168	3.17777942283339 \\
-4.75465693156259	3.08076239080349 \\
-4.74943076508912	2.98169746295654 \\
-4.68986873189466	3.02819436996338 \\
-5.22402694889216	3.2277786117442 \\
-5.3174752536479	2.95332607094287 \\
-5.49536633547493	3.36887739686349 \\
-5.85809121676369	3.34731239722109 \\
-6.30146934501843	2.91878797949146 \\
-6.38092935825125	3.65164737005277 \\
-6.18680660476561	3.67401442836873 \\
-6.26593169494411	3.55567828877746 \\
-6.32209439598457	3.27633942117678 \\
-6.40559753029272	3.18678204285194 \\
-6.55560886574131	3.32506139752787 \\
-6.58802252355008	2.84036322196304 \\
-6.40811024390267	2.66152049008635 \\
-6.20891366258093	2.53514651064497 \\
-6.16916917397692	2.53480266883758 \\
-6.62783133166524	2.49926972605076 \\
-6.76505459404285	1.93999249733266 \\
-6.70900791506967	1.86252569078329 \\
-6.99461145627245	1.80829252833306 \\
-7.25159971691313	1.68741150094702 \\
-6.88585755203886	2.1751301716828 \\
-7.03298224775347	2.22578864081615 \\
-6.39009927292675	2.26489708570827 \\
-5.97147506961428	2.27659473399206 \\
-5.85891405622394	2.27148926835951 \\
-5.45264199359012	2.42107775094772 \\
-5.47235483744656	2.70731015434488 \\
-5.56729651817912	2.60784442034656 \\
-5.30953913328056	2.88535717260394 \\
-5.26530915574587	2.76538541535435 \\
-5.45126933234049	2.63753543460764 \\
-5.29393153657098	2.30366167515297 \\
-5.04233775667337	2.29648753763484 \\
-5.25477474836798	2.70153032931035 \\
-5.1961803212118	3.00802727629842 \\
-5.67730212313656	3.38580510813035 \\
-5.77044370882654	3.26910417191648 \\
-5.56273740692767	3.41741883685151 \\
-5.59238811138251	3.76646831510492 \\
-5.77604057397689	3.91370997262956 \\
-5.66231314835848	4.13740636212 \\
-5.97604368833547	4.03183732483556 \\
-5.41149117022914	3.85301053283955 \\
-5.47645735458477	3.60199460765058 \\
-5.94546418499113	4.06515938102757 \\
-6.06597084402999	4.10163552945563 \\
-5.67519439994425	3.98356078915408 \\
-5.07135047889738	4.11258511102718 \\
-5.61819006575155	3.81256450153485 \\
-5.54358327389878	4.06564153983422 \\
-5.54381778455484	3.75359611976085 \\
-5.66861270778044	4.01620095340151 \\
-5.96128337657702	4.08162559310317 \\
-6.37269419917811	4.10972143971034 \\
-5.86248689367971	4.2423799485537 \\
-5.67400187574217	4.47146232484995 \\
-5.7461924668047	4.53903009459488 \\
-5.72742474595925	4.486512647276 \\
-6.0217420536144	4.32172072931142 \\
-5.78150209702125	4.4477136291484 \\
-5.55434628324072	4.56297799794228 \\
-5.47055185018359	4.65615184805981 \\
-5.05086465133419	4.62738817073836 \\
-4.8571094619363	4.35739930498405 \\
-5.2142073623958	4.34186581210019 \\
-5.50975768799994	4.3923511082342 \\
-5.55158626589626	4.5216176131749 \\
-5.68704983609499	4.57418838316185 \\
-5.53211434364763	4.78011824929023 \\
-5.86300235383969	4.85899627708092 \\
-5.80794261969384	5.30525112233418 \\
-5.97168795033882	5.12481746567657 \\
-5.7085126910693	5.59910539476824 \\
-5.42950325554284	5.95333603344721 \\
-5.25634848903944	6.17801827729679 \\
-5.06719171703309	6.34190259680219 \\
-5.27150453529264	6.29731712395395 \\
-5.18419803428914	6.40959112574838 \\
-4.91199759169732	6.3912304239219 \\
-5.29580585258898	6.36448502784216 \\
-5.14599504795809	6.27207429957223 \\
-5.26287860852561	6.33960088784014 \\
-4.95890286321674	6.29897137037662 \\
-4.3443199013254	6.3910259904563 \\
-4.74721197117429	6.48217064946343 \\
-4.78499033501166	6.97725658117631 \\
-4.86875918708758	6.67729640118303 \\
-4.95798718353626	6.85546873066564 \\
-4.88766416727469	7.06191430834812 \\
-4.90138575464664	7.24554806923935 \\
-5.31389781692285	7.80144406799576 \\
-5.05682994745677	7.80830959503223 \\
-4.83584327882168	7.88135195528532 \\
-4.65636024156219	8.24256109385775 \\
-4.71616851190341	8.25253133499895 \\
-4.46576551049985	8.54991666281245 \\
-4.30675813180824	8.45407737029916 \\
-4.02161761911288	8.59797025322452 \\
-4.06370524183021	8.65127920996432 \\
-4.3923020037959	9.27521332780324 \\
-4.28783625066728	9.43154437470182 \\
-4.75255015686233	9.2367916752061 \\
-4.87137337929061	9.04981648444848 \\
-4.97426929084139	9.30168163222554 \\
-5.09861726325704	9.49094523871645 \\
-5.34250545657659	9.57250068153911 \\
-5.36529220595574	9.69551680062377 \\
-5.56091259424924	9.8933567392083 \\
-5.41429703916493	9.69560285537208 \\
-5.3195700908654	10.1034559289205 \\
-5.36252464643283	9.88388913021921 \\
-5.39238257502974	10.1533658512582 \\
-5.33903754578897	10.1864395320701 \\
-4.96432770914669	10.0144717049694 \\
-4.4395010193241	9.99027094278272 \\
-4.49875177403482	10.0884657072151 \\
-4.81812512568532	9.83518075710829 \\
-4.8234160320712	9.75893167243059 \\
-5.08458261559986	9.49385016653969 \\
-4.97744749724374	9.7282412530844 \\
-5.17076280193868	9.64670240213831 \\
-5.08470585126252	10.0147570582991 \\
-5.09017222845696	10.1359836093175 \\
-4.69049218025341	10.0874922779158 \\
-4.8864833289665	9.6671567010078 \\
-4.32006246159325	9.55086771823254 \\
-4.17483811132758	8.93712003263629 \\
-4.14398105606526	8.90548129307442 \\
-4.11690148516444	9.16790659942947 \\
-4.12673028847339	9.52188878690674 \\
-4.01323680991956	9.98913927748194 \\
-3.38229209754965	10.2495286490123 \\
-3.3935144703023	10.1105815428653 \\
-3.4369460629612	10.7735533572381 \\
-3.58863075092971	10.9425331311128 \\
-3.44160972427293	10.828784824191 \\
-3.56683083264258	10.6073803597628 \\
-3.66144359486705	10.8036513855291 \\
-3.7771259668387	11.0557423139291 \\
-3.38051880261596	11.5273821890265 \\
-3.39465447140425	11.8750335086439 \\
-3.32244534987273	12.0645888770623 \\
-3.06957046310642	12.0699713960554 \\
-2.82656964162042	11.7927192660806 \\
-3.03651232521086	12.0339649077605 \\
-3.08153010145504	12.3738893277857 \\
-2.97149813266578	12.4186425487678 \\
-2.88206629672443	12.2058611820957 \\
-2.83620964426078	12.1827061147751 \\
-2.8603081675003	12.0503727203128 \\
-2.95807286299234	12.0012049655527 \\
-2.86578334311143	11.653905887697 \\
-3.10259173562418	11.7814740946981 \\
-3.24346503728899	11.9881651776565 \\
-3.14184794532276	12.1655526853388 \\
-3.26425875348496	11.9760401967506 \\
-3.37338544706672	12.3185681214001 \\
-3.20500826241897	12.3115974683891 \\
-3.27273046250428	12.2894354415156 \\
-3.10511031309652	12.0141777596014 \\
-3.20574987035156	11.9106635571361 \\
-3.40297683294199	12.1245005952553 \\
-3.28136226157364	12.2930970855178 \\
-3.08514783227649	12.2468669971295 \\
-3.16469072966945	12.6664698590241 \\
-2.6848998635369	12.0540292549241 \\
-2.57898771062921	11.774450904076 \\
-2.42407050570584	12.0731470372812 \\
-2.19391131938353	12.2408894327251 \\
-2.35015313341061	12.6587940611408 \\
-2.69160629353026	12.5993113100753 \\
-2.48429729580023	11.6655552080407 \\
-2.47274077045137	11.7801472059185 \\
-2.76447626114531	11.5713897101894 \\
-2.55982922377415	11.3530200412535 \\
-2.70606955408296	11.290975592206 \\
-3.11403834403887	10.8489522347466 \\
-3.16722824995776	10.6135868061976 \\
-3.8497943542572	10.3900355687733 \\
-3.75713213242138	10.7024972603347 \\
-3.69312969395506	10.8281584362012 \\
-3.49781643943444	10.5617311363724 \\
-3.93206068702345	11.0042070619853 \\
-4.09496333409647	10.8185463251961 \\
-3.84376605749667	10.7156726846058 \\
-3.97280542105128	10.4877090060226 \\
-3.78047921380504	10.266102445137 \\
-3.95445554183943	10.0387528475004 \\
-3.55919605828502	10.23826723212 \\
-3.88941437787855	10.0103091423037 \\
-3.90058919489425	10.0121138748039 \\
-4.07127394494419	9.93296593903152 \\
-3.96696589098292	9.99944773256254 \\
-4.0089542648522	9.6996128690491 \\
-3.70433284089608	9.55029076321349 \\
-3.45162851618936	9.47964872360351 \\
-3.54771522721206	9.23268415815502 \\
-3.55842829089925	9.18454362977815 \\
-3.13200637228376	8.77853197919712 \\
-3.25872692406696	8.62835066647932 \\
-3.08808697224603	8.49175096687732 \\
-2.93926021813267	8.7613977878944 \\
-2.99435581580731	8.51232330942018 \\
-3.16362161069893	8.47985080199019 \\
-3.48124348727949	8.49269628622627 \\
-3.49047836892924	8.97220671940495 \\
-3.44389581228536	9.26488348522881 \\
-3.23969180801275	9.25694178355968 \\
-3.44173855226425	9.2311302983016 \\
-3.1768612954031	9.55594177502273 \\
-2.91187273700847	9.73121390853797 \\
-3.0994315417649	9.75696379143916 \\
-2.97093442843451	9.87139543143922 \\
-2.70302779450563	9.84921418708401 \\
-2.91497514316175	9.64252868154884 \\
-2.59400227834236	9.54961849569853 \\
-3.23169807556575	9.48544338124094 \\
-3.31963444827152	9.38947032713028 \\
-3.24395448302022	9.10254397411756 \\
-3.30733533587927	9.12097239605393 \\
-3.19883850354246	9.18688030843051 \\
-3.68057873746999	9.22201849276287 \\
-3.47866088306175	9.25254394909602 \\
-3.65867006032425	9.24274519954408 \\
-3.66755002898408	9.57844555934432 \\
-3.79486588347383	9.50276421602368 \\
-4.28265435035769	9.93074961027579 \\
-4.20547019742274	9.92832496581453 \\
-4.27489684671092	9.84989821591825 \\
-4.50139165909652	9.67902965098152 \\
-4.24812513623494	9.99342824401638 \\
-4.62809656704944	10.0715878054379 \\
-4.89300009802354	10.3286022708433 \\
-4.91863941247246	10.2178077187691 \\
-5.00735759575445	10.0840548901221 \\
-4.51163084330684	10.0529270807549 \\
-4.70162794200998	9.96635851412625 \\
-4.92519615950537	9.48176247786684 \\
-4.98094572868311	9.56859322357541 \\
-4.79658982638852	10.1693334153154 \\
-4.95454035280329	10.2795425938683 \\
-4.72185837757509	10.003799770576 \\
-4.66582272374419	9.96112661893113 \\
-5.07785410498443	9.80958681568541 \\
-5.21249104545648	10.1430330383959 \\
-4.89681771576362	10.1070628501443 \\
-4.53592062198468	10.4759689585283 \\
-4.2971995507254	9.86993392018876 \\
-4.14874338011652	9.60023336062658 \\
-4.36137642905112	9.86565263033095 \\
-3.95069796533597	9.51355954538884 \\
-3.82661806448053	9.60774533068137 \\
-3.65727574925362	9.48007770467841 \\
-3.43832686522281	9.60275715191419 \\
-3.5584736412731	9.68661124448871 \\
-3.48008780802625	9.57451429209269 \\
-3.50678217154379	9.71149106166362 \\
-3.99425900133378	10.1027161586665 \\
-3.92489968655018	9.91458077567547 \\
-4.27172812022789	9.82447875033574 \\
-4.4732936827075	10.2623200283566 \\
-4.50607058987192	10.4143553791915 \\
-4.07661541473509	10.4205285394463 \\
-4.14288933671001	10.3319526524382 \\
-3.58874445784546	10.7077440138511 \\
-3.83519275562423	10.6368872710342 \\
-3.81868225260248	10.5704549081782 \\
-3.42219570143317	10.480380586925 \\
-3.28199818988798	9.9855971352403 \\
-3.11356282405065	10.026934187299 \\
-2.71083297563867	10.1602759509021 \\
-2.56993887472008	10.0503052972145 \\
-2.1609843302859	9.85753241706682 \\
-2.07297386805753	9.85191991104373 \\
-2.59553339043151	10.0398061388781 \\
-2.59108418803933	10.2084229468094 \\
-3.28553354151942	10.1010178462329 \\
-3.18008203126871	10.2944408667364 \\
-2.88961803251831	10.1488449032467 \\
-3.03250901161929	9.97489239112799 \\
-2.82820730423084	10.9482062071694 \\
-2.90337301028778	10.6465766845941 \\
-3.07608604979354	10.0395161551992 \\
-3.18766207190206	10.0303011915743 \\
-2.9636301655422	10.0731645330333 \\
-3.21951469339689	10.1651311536657 \\
-3.18554547940272	10.2453643213614 \\
-3.17124771110643	10.3355751944356 \\
-3.29873630494123	10.1324735645534 \\
};

\end{axis}

\end{tikzpicture}
